Advancing Reliable Synthetic Video Detection: Insights from the SAFE Challenge

The proliferation of generative video technologies has intensified the need for reliable methods to detect and characterize synthetic media. To address this challenge, we organized the \href{https://safe-video-2025.dsri.org}{SAFE: Synthetic Video Detection Challenge}, co-located with the \textit{Authenticity and Provenance in the Age of Generative AI (APAI) Workshop }at ICCV 2025. The competition invited participants to develop and evaluate algorithms capable of distinguishing real from synthetic videos under fully blind evaluation conditions with over 600 submissions from 12 teams over a 90 day span. Hosted on the Hugging Face platform, the challenge comprised two primary tasks: (1) detection of synthetic video content generated by diverse state-of-the-art models, and (2) detection of synthetic content following common post-processing operations such as resizing, re-compression, motion blur and others. The challenge data consisted of 13 modern high quality synthetic video models with generated content matched to real videos from 21 diverse and challenge sources, all adding up to 20 hours of 6,000 video samples. This paper describes the challenge design, dataset construction, evaluation methodology, and outcomes, offering insights into the generalization and robustness of contemporary synthetic video detection methods. Our findings highlight measurable progress in cross-generator generalization but also persistent vulnerabilities to post-processing artifacts. https://safe-video-2025.dsri.org

==> tables/top6_tasks.tex <==
\begin{table*}[tb]
\centering
\caption{Comparison of the top six teams...}
\label{tab:top6_tasks}

\begin{tabular}{lcccccc}
\toprule
\textbf{Team} &
\multicolumn{3}{c}{\textbf{Task~1: Original Content}} &
\multicolumn{3}{c}{\textbf{Task~2: Post-Processed Content}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
 & \textbf{TPR} & \textbf{TNR} & \textbf{BAC} & \textbf{TPR} & \textbf{TNR} & \textbf{BAC} \\
\midrule
\textbf{GRIP-UNINA} & 0.84 & 0.88 & \textbf{0.86} & 0.66 & 0.82 & \textbf{0.74} \\
\textbf{ISPL-Realynx} & 0.86 & 0.84 & \textbf{0.85} & 0.82 & 0.59 & \textbf{0.70} \\
\textbf{DASH} & 0.77 & 0.90 & \textbf{0.84} & 0.71 & 0.75 & \textbf{0.73} \\
\textbf{Lemma1727} & 0.79 & 0.87 & \textbf{0.83} & 0.74 & 0.66 & \textbf{0.70} \\
\textbf{Truebees} & 0.66 & 0.88 & \textbf{0.77} & 0.59 & 0.73 & \textbf{0.66} \\
\textbf{Shahidmuneer} & 0.77 & 0.76 & \textbf{0.77} & 0.54 & 0.53 & \textbf{0.54} \\
\bottomrule
\end{tabular}
\caption{Comparison of the top six teams...}
\label{tab:top6_tasks}
\end{table*}
